Stanley's character polynomials and coloured factorizations in the symmetric group

Stanley introduces polynomials which help evaluate symmetric group characters and conjectures that the coefficients of the polynomials are positive. Stanley later gives a conjectured combinatorial interpretation for the coefficients of the polynomials. Here, we prove the conjecture for the terms of highest degree.

==> thmstuff.tex <==
%theorems, lemmas and things like that

\theoremstyle{plain}
\RequirePackage{latexsym}
%\theoremsymbol{\ensuremath{\Box}}
\theoremseparator{.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% basic theorem environments

\newtheorem{theorem}{Theorem}[section]
\newtheorem{cor}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{prop}[theorem]{Proposition}
\newtheorem{notation}{Notation}
\newtheorem{defn}{Definition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{proposition}[theorem]{Proposition}

{\theorembodyfont{\normalfont} \theoremsymbol{\ensuremath{\Box}}
\newtheorem{example}[theorem]{Example}}
{\theorembodyfont{\normalfont} \theoremsymbol{\ensuremath{\Box}}
\newtheorem{remark}{Remark}}
{\theorembodyfont{\normalfont} \newtheorem{quest}{Question}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%proof environment

\theoremstyle{nonumberplain}
\theoremheaderfont{\it}
\theorembodyfont{\normalfont}
\RequirePackage{latexsym}
\theoremsymbol{\ensuremath{\Box}}
\RequirePackage{amssymb}
\newtheorem{proof}{Proof}

%proof of environment

\theoremstyle{empty}
\theoremheaderfont{\bf}
\theorembodyfont{\normalfont}
\RequirePackage{latexsym}
\theoremsymbol{\ensuremath{\Box}}
\RequirePackage{amssymb}
\newtheorem{proofof}{Proof}


%margin size
\setlength{\hoffset}{-1in}              %`driver' margin
\setlength{\voffset}{-0.75in}           %`driver' margin
\setlength{\textwidth}{5.5in}           %width of text body
\setlength{\textheight}{8.5in}            %height of text body
\setlength{\evensidemargin}{1.5in}        %driver margin to body
\setlength{\oddsidemargin}{1.5in}         %driver margin to body
%\setlength{\topmargin}{0in}             %from driver margin to header
%\setlength{\marginparwidth}{0pt}
%\setlength{\marginparsep}{0pt}         %horizontal space between
%\setlength{\marginparpush}{0pt}        %min space between par
%\setlength{\headsep}{0pt}
%\setlength{\headheight}{0pt}
\setlength{\footskip}{0.5in}
%\setlength{\linewidth}{0pt}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%solution environment

\theoremstyle{nonumberplain}
\theoremheaderfont{\it}
\theorembodyfont{\normalfont}
\RequirePackage{latexsym}
\theoremsymbol{\ensuremath{\Box}}
\RequirePackage{amssymb}
\newtheorem{sol}{Solution}

%margin size
\setlength{\hoffset}{-1in}              %`driver' margin
\setlength{\voffset}{-0.75in}           %`driver' margin
\setlength{\textwidth}{5.5in}           %width of text body
\setlength{\textheight}{8.5in}            %height of text body
\setlength{\evensidemargin}{1.5in}        %driver margin to body
\setlength{\oddsidemargin}{1.5in}         %driver margin to body
%\setlength{\topmargin}{0in}             %from driver margin to header
%\setlength{\marginparwidth}{0pt}
%\setlength{\marginparsep}{0pt}         %horizontal space between
%\setlength{\marginparpush}{0pt}        %min space between par
%\setlength{\headsep}{0pt}
%\setlength{\headheight}{0pt}
\setlength{\footskip}{0.5in}
%\setlength{\linewidth}{0pt}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Local Variables: 
%%% mode: plain-tex
%%% TeX-master: "thmstuff"
%%% End: 

